Kinematics and Thermodynamics of Coronal Mass Ejections

Coronal mass ejections (CMEs) are major drivers of space weather, yet their thermodynamic evolution remains insufficiently constrained. This thesis develops a comprehensive framework linking CME kinematics, thermodynamics, internal force balance, and geoeffectiveness through analytical modelling and multi-viewpoint observations. The developed FRIS model uses observed kinematics to infer otherwise inaccessible internal plasma properties, including the polytropic index. A systematic investigation of fast CMEs reveals an initial heat-release phase followed by a transition towards near-isothermal evolution, typically around 3-9 solar radii. The evolving contributions of thermal-pressure and centrifugal forces, opposed by the Lorentz force, establish a connection between expansion and thermal evolution. The findings demonstrate the limitations of assuming a fixed polytropic index in magnetohydrodynamic models of CME propagation. At 1 au, in situ observations reveal persistent non-adiabatic evolution, accompanied by turbulence and localised intermittency. The interacting CMEs associated with the May 2024 great storm show restructured magnetic and thermal configurations, producing double-flux-rope-like signatures and species-dependent heating, with electron thermodynamics as a better indicator of recent interactions. Statistical analysis of nearly 600 ME demonstrates that 45% exhibit net heating with a solar cycle dependence. Notably, High-impact ejecta preferentially exhibit stronger heating signatures, establishing thermal state as a complementary diagnostic of geoeffectiveness. Overall, this thesis establishes CMEs as intrinsically non-adiabatic systems whose thermodynamic evolution is coupled to expansion, internal force balance, solar-cycle variability, and CME-CME interactions, with important implications for understanding geoeffectiveness and improving space-weather assessment.

==> Prologue/Abbreviations.tex <==
\lhead{\emph{Abbreviations}}  
\listofsymbols{ll} 
{

}

\clearpage
\thispagestyle{empty}
\newpage





==> Prologue/data_software.tex <==
\textit{\huge Software usage}\\
\\

\begin{description}
    \item[Data Reduction:] Throughout this work, various data reduction software have been used extensively. These are utilized to reduce data covering ultraviolet to infrared bands and are as follows: \texttt{IRAF} \citep{93_tody}, \texttt{PyRAF}, \texttt{HEASoft}  \citep{2014ascl.soft08004N}, \texttt{ds9} \citep{2000ascl.soft03002S}, \texttt{CCDLAB} \citep{2017PASP_postma}, \texttt{UVOTPY} \citep{2014ascl.soft10004K}.

    \item[Light Curve \& Spectra Modeling:] This work also utilizes 1-D stellar evolution software \texttt{MESA} (r-15140) \citep{Paxton2011, Paxton2013, Paxton2015, Paxton2018, Paxton2019} , multi-group radiation-hydrodyanmics software \texttt{STELLA} \citep{Blinnikov2004, Baklanov2005, Blinnikov2006}, and synthetic spectral generation software \texttt{SYNAPPS} \citep{2011PASP..123..237T}.

    \item[Analysis:] For most of the analysis and figures presented in this thesis, various \textit{Python} libraries have been used. Some of the key packages are: \textit{astropy} \citep{astropy:2013, astropy:2018, astropy:2022},
\textit{emcee} \citep{2013PASP..125..306F},
\textit{Jupyter-notebook} \citep{jupyter},
\textit{matplotlib} \citep{Hunter:2007},
\textit{numpy} \citep{harris2020array},
\textit{pandas} \citep{mckinney-proc-scipy-2010, reback2020pandas},
\textit{scipy} \citep{2020SciPy-NMeth},
\textit{seaborn} \citep{Waskom2021} 

\item[Others:] Various resources available online such as ADS, WISeREP \citep{2012yaron}, Open Supernova Catalog \citep{2017guillochon}, ALeRCE \citep{2021Alerce}, ATLAS \citep{2018tonry}, and SVO FPS \citep{SVO2} have also been utilized. Related data files (photometry, spectroscopy, models) are available online. \textit{Other data/scripts/jupyter-notebooks used in this work are made available on my personal website:\\ \href{https://astronomoid.github.io}{astronomoid.github.io} and Github account \href{https://github.com/Astronomoid}{github.com/Astronomoid}}
\end{description}

==> Prologue/publications.tex <==

\vspace*{0.7cm}
\begin{center}
{\huge\bf List of Publications}
\end{center}
\vspace{0.7cm}

%\setcounter{page}
%{\large \bf \it Publications included in this thesis}
%\vspace{-0.5cm}
\begin{enumerate}[leftmargin=0pt]

    \item \textbf{Erratum: Modeling the Thermodynamic Evolution of Coronal Mass Ejections Using Their Kinematics (2018, ApJ, 865, 50)}, 2023, Wageesh Mishra, Yuming Wang, Shaoyu Lyu and {\bf \textcolor{orange!70!black}{Soumyaranjan Khuntia}}, \textit{\textbf{The Astrophysical Journal}, Volume 952, Number 2, Page 173,} \href{http://doi.org/10.3847/1538-4357/ace691}{DOI:10.3847/1538-4357/ace691}


    \item \textbf{Unraveling the Thermodynamic Enigma between Fast and Slow Coronal Mass Ejections}, 2023, {\bf \textcolor{orange!70!black}{Soumyaranjan Khuntia}}, Wageesh Mishra, Sudheer K. Mishra, Yuming Wang, Jie Zhang, and Shaoyu Lyu, \textit{\textbf{The Astrophysical Journal}, Volume 958, Number 1, Page 92,} \href{http://doi.org/10.3847/1538-4357/ad00ba}{DOI:10.3847/1538-4357/ad00ba}


    \item \textbf{Distribution and Recovery Phase of Geomagnetic Storms During Solar Cycles 23 and 24}, 2024, Wageesh Mishra, Preity Sukla Sahani, {\bf \textcolor{orange!70!black}{Soumyaranjan Khuntia}} and Dibyendu Chakrabarty, \textit{\textbf{Monthly Notices of the Royal Astronomical Society}, Volume 530, Issue 3, Page 3171,} \href{https://doi.org/10.1093/mnras/stae1045}{DOI: 10.1093/mnras/stae1045}
   
    
    \item \textbf{Deciphering the Evolution of Thermodynamic Properties and their Connection to the Global Kinematics of High-speed Coronal Mass Ejections using FRIS Model}, 2024, {\bf \textcolor{orange!70!black}{Soumyaranjan Khuntia}}, Wageesh Mishra, Yuming Wang, Sudheer K. Mishra, Teresa Nieves-Chinchilla and Shaoyu Lyu, \textit{\textbf{Monthly Notices of the Royal Astronomical Society}, Volume 535, Issue 3, Page 2585,} \href{https://doi.org/10.1093/mnras/stae2523}{DOI: 10.1093/mnras/stae2523}

    \item \textbf{Evolution of the Interacting Coronal Mass Ejections that Drove the Great Geomagnetic Storm of 10 May 2024}, 2025a, {\bf \textcolor{orange!70!black}{Soumyaranjan Khuntia}}, Wageesh Mishra, and Anjali Agarwal, \textit{\textbf{Astronomy and Astrophysics}, Volume 698, Article Number A79, Pages 14,} \href{https://doi.org/10.1051/0004-6361/202452866}{DOI: 10.1051/0004-6361/202452866}
    
\end{enumerate}

\vfill
\hfill \textit{Continued on next page}


%\clearpage\null\newpage
\clearpage\null

\begin{enumerate}[leftmargin=0pt]
\setcounter{enumi}{5}
    \item \textbf{Thermal and Turbulence Characteristics of Fast and Slow Coronal Mass Ejections at 1 AU}, 2025b, {\bf \textcolor{orange!70!black}{Soumyaranjan Khuntia}} and Wageesh Mishra, \textit{\textbf{Journal of Astrophysics and Astronomy}, Volume 698, Article Number A79, Pages 14,}\\ \href{https://doi.org/10.1051/0004-6361/202452866}{DOI: 10.1051/0004-6361/202452866}

    \item \textbf{Statistical Analysis of the Thermal State of Interplanetary Coronal Mass Ejections at 1 AU in Connection to their Geoeffectiveness Over Solar Cycle 23-25}, 2025c, {\bf \textcolor{orange!70!black}{Soumyaranjan Khuntia}} and Wageesh Mishra (\textit{Under review})
 
\end{enumerate}


% \vspace{2cm}
% {\large \bf \it B) Contributed publications [Not part of this thesis]}
% %\vspace{-0.7cm}
% \begin{enumerate}[leftmargin=0pt]
%     \item \textbf{Thermal analysis of sub-alfvenic regions in Solar Wind Structures}; Komal Choraghe, Wageesh Mishra and {\bf \textcolor{orange!70!black}{Soumyaranjan Khuntia}} (\textit{Under review})

%      \item \textbf{Asymmetric expansion of coronal mass ejections}; Anjali Agarwal, Wageesh Mishra and {\bf \textcolor{orange!70!black}{Soumyaranjan Khuntia}} (\textit{Under review})
    
% \end{enumerate}

